Multiscale Simulations of Complex Systems by Learning their Effective Dynamics

Predictive simulations of complex systems are essential for applications ranging from weather forecasting to drug design. The veracity of these predictions hinges on their capacity to capture the effective system dynamics. Massively parallel simulations predict the system dynamics by resolving all spatiotemporal scales, often at a cost that prevents experimentation while their findings may not allow for generalisation. On the other hand reduced order models are fast but limited by the frequently adopted linearization of the system dynamics and/or the utilization of heuristic closures. Here we present a novel systematic framework that bridges large scale simulations and reduced order models to Learn the Effective Dynamics (LED) of diverse complex systems. The framework forms algorithmic alloys between non-linear machine learning algorithms and the Equation-Free approach for modeling complex systems. LED deploys autoencoders to formulate a mapping between fine and coarse-grained representations and evolves the latent space dynamics using recurrent neural networks. The algorithm is validated on benchmark problems and we find that it outperforms state of the art reduced order models in terms of predictability and large scale simulations in terms of cost. LED is applicable to systems ranging from chemistry to fluid mechanics and reduces the computational effort by up to two orders of magnitude while maintaining the prediction accuracy of the full system dynamics. We argue that LED provides a novel potent modality for the accurate prediction of complex systems.

==> section-AD-1D.tex <==
% !TEX root =./SI_PNAS.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     AD - 1D
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Advection-Diffusion with Brownian dynamics 1-D}
\label{app:sec:dif1d}

In this section, we evaluate LED on a system of $N$ point particles on a bounded domain $\Omega = \left[-L/2, L/2\right]^{d_{\bmx}}$, where $d_{\bmx}$ is the dimension of the space, whose dynamics are determined by the advection-diffusion equation, modeled with the stochastic differential equation (SDE)
%
\begin{equation} 
d\bm{x}_t = \bm{u}(t) dt + \sqrt{D} \, d\bm{W}_t,
\label{eq:app:SDE}
\end{equation}
%
where $\bmx_t \in \Omega$ denotes the position of the particle at time $t$, $D \in \mathbb{R}$ is the diffusion coefficient, $d\bm{W}_t \in \mathbb{R}^{d_{\bmx}}$ is a Wiener process, and $\bm{u}(t) = \bm{A} \cos( \bm{\omega} t) \in \mathbb{R}^{d_{\bmx}}$ is a cosine advection (drift) term.
\Cref{eq:app:SDE} is solved with initial conditions $\bmx_0 = \bm{0}$ and reflective boundary conditions, ensuring that $\bmx_t \in \Omega, \forall t$.
The system is advanced in time with explicit Euler integration.
We pick a domain size of $L=1$.
In this section, we consider the one dimensional case with $d_{\bmx}=1$.
We solve for $N=1000$ particles, and consider the values $D=0.2$, $A=1$ and $\omega =0.1$.
The stochastic dynamics are solved with a time-step $\delta t=10^{-3}$.
By saving the positions of the particles at a coarser  time-step $\Delta t = 0.5$ and starting from different random initial conditions, we generate three datasets, a training and a validation dataset, each consisting of $10^3$ samples, and a test dataset with $10^4$ samples.
\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{AD-1D-iterative_latent_forecasting_test_2780_density_contour.pdf}
\caption{
LED applied on the one dimensional Advection-Diffusion equation.
The dimensionality of the latent dimension of the VAE is $d_{\bmz}=1$.
LED successfully uncovered the cosine dynamics on the latent space, even though the dimensionality of the original state $\bms_t$ describing the state of the system $\bms_t \in \mathbb{R}^{N}$, with $N=1000$.
However, due to the iterative propagation of the latent dynamics with LED, a phase lag is introduced, making the error to increase with time.
This can be seen for example, in the error on the estimated mean position (M1) of the particles.
Nevertheless, the variance is captured along with the long-term statistical behavior.
}
\label{fig:app:AD-1D:iterative_latent_forecasting_test_2780_density_contour}
\end{figure}
We trained a VAE with permutation invariant input layer, a latent dimension $d_{\bmz}=1$, and a mixture density decoder to compress the dynamics.
Then, we trained the RNN of LED to forecast the one-dimensional latent dynamics.
The result of an iterative prediction on the test dataset is given in~\Cref{fig:app:AD-1D:iterative_latent_forecasting_test_2780_density_contour}.
The warm-up period of LED is set to $T_{warm}=60$.
The network is fed an initial configuration of particles $\bms_t=[x^1_t, \dots, x^N_t ]^T \in \mathbb{R}^N$, compresses the configuration to one number $z_t \in \mathbb{R}$, and utilizes the RNN to forecast the next latent dynamics $\bmz_{t+1}$.
From this latent space, the MD decoder of LED is sampling the next configuration $\bms_{t+1}$.
LED successfully uncovered the inherent cosine dynamics of the stochastic movement of the particles, even though the dimensionality of the reduced order space was very low ($d_{\bmz}=1$).
We plot the L1-NHD error between the predicted and true density of particle positions, along with the Wasserstein distance and the error on the first two moments on the particle positions as a function of time.
From the low dimensional latent space, the decoder of LED learned to map to the position of the $N=1000$ particles, as depicted by the low error on the densities.
As expected, due to the iterative propagation of the model error, the prediction diverges and there is a phase lag between the predicted and the true dynamics.
This causes an increase of the error on the estimated mean position of the particles (M1) and an error on the variance (M2).
Even though the error on the variance is kept low, the error on M1 is increasing as we iteratively forecast for a large horizon.


Regarding the hyper-parameters of LED, we tune them based on a grid search reported in~\Cref{app:sec:ad1d:hyperparams}.
The inputs to the network are scaled to $[0,1]$, while adding noise in the input did not improve performance for this case.
Performance is measured in terms of the maximum data likelihood of the MD autoencoder, and the minimum root mean square error for the RNN part, which are trained independently.
The autoencoder with the highest likelihood from our grid search, turned out to be a VAE, with a permutation invariant input layer  (function $\phi$ in~\Cref{fig:permInvLayer}) consisting of $5$ residual layers of $100$ nodes and $\tanh$ activation, mapping to a permutation invariant latent space of dimension $M=200$ with mean feature function, with an additional residual autoencoder (modeling function $g$ in~\Cref{fig:permInvLayer})  with $5$ layers of $100$ hidden nodes each and $\tanh$ activation, reducing the dimensionality to a latent space of dimension $d_{\bmz}=1$.
Finally, the decoder is composed of $5$ additional residual layers of $100$ size each, and a mixture density output layer, with $50$ hidden units, and $4$ kernels outputting the parameters for the mixture coefficients, the means, and the covariance matrices of the $4$ kernels.
A configuration can be sampled in a trivial way from this representation.
Regarding the RNN part of LED, a stateful LSTM with 1 layer of $100$ nodes trained with a BBTT truncated length of $100$ exhibited the lowest validation error.
%# |      1 | 0.6717 |          0.0128 |     0.0318 |     0.0038 |     0.0072 | None        | None        | GPU-ARNN-N_used_2000-N_20000-scaler_MinMaxZeroOne-NL_0-LR_0.001-L2_0.0001-VAR_1-MDN_normal-KERN_4-HIDDEN_50-PERM_INV_200-FEAT_mean-AUTO_5x100-ACT_tanh-RES_1-DKP_1-LD_1-C_lstm-ACT_tanh-RNN_1x100-ITLL_0-SL_100 |

In the following, we employ LED to perform multiscale forecasting switching between propagation of the latent dynamics for $T_{m}=450$ and evolution of the particle dynamics for $T_{\mu}=50$, leading to a multiscale ratio of $\rho=T_{m}/T_{\mu}=9$.
The initial warm-up period of LED is $T_{warm}=60$.
The iterative propagation on the test set is plotted in~\Cref{fig:app:AD-1D:multiscale_forecasting_micro_100_macro_900_test_2780_density_contour}.
We observe that by switching to the particle configuration and evolving the dynamics, we alleviate the iterative error propagation, at the additional cost of propagating the original system dynamics (Brownian motion of the $N=1000$ particles) for $10\%$ of the total time.
The statistics of the system are captured well as demonstrated by the low error on the L1-NHD, the mean (M1) and variance (M2) of the particles.
\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{AD-1D-multiscale_forecasting_micro_100_macro_900_test_2780_density_contour.pdf}
\caption{
Multiscale LED applied on the one dimensional Advection-Diffusion equation, switching between the propagation of the latent space dynamics for $T_{m}=450$, and evolution of the particle dynamics for $T_{\mu}=50$.
The dimensionality of the latent dimension of the VAE is $d_{\bmz}=1$.
The particle dynamics are correcting the error in the phase lag introduced by the iterative propagation on the latent space.
}
\label{fig:app:AD-1D:multiscale_forecasting_micro_100_macro_900_test_2780_density_contour}
\end{figure}







\iffalse
\subsubsection{Statistical Analysis}
\label{app:sec:ad1d:statanal}

In this section, we perform a statistical analysis to evaluate the performance of LED in forecasting the stochastic dynamics of a group of $N=1000$ particles whose dynamics are governed by the Advection-Diffusion equation.
Starting from $20$ different initial conditions, we propagate the dynamics with LED $400$ different times, changing the seed up to a final time of $T_f=4000$, which is equivalent to $8000$ steps.
Since LED is sampling from the MD decoder, every run will result to a different evolution of the configuration, as expected.
For every run, we calculate the first two moments of the configuration, M1 and M2.
At each time-step, we have $400$ predicted M1 and M2.
In order to evaluate the statistical error, we compare the predicted distributions of M1 and M2, with the groundtruth one, by evaluating their L1-NHD and the WD.
The evolution of these errors as a function of time is plotted in~
\Cref{fig:app:AD-1D:statistical_analysis_1} for four variants of LED with different $T_{m}$.
The initial warm-up period of LED is $T_{warm}=60$.
Note that as we decrease $T_m$, i.e. the time spent evolving the latent dynamics of LED, all error metrics decrease.
\begin{figure*}[tbhp]
\centering
\begin{subfigure}[tbhp]{0.4\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{AD-1D-StatComparison_batchfiles_200_test_legend.pdf}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[tbhp]{0.6\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{AD-1D-StatComparison_batchfiles_200_test_L1_hist_error_M_1_evol.pdf}
%\caption{}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[tbhp]{0.6\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{AD-1D-StatComparison_batchfiles_200_test_L1_hist_error_M_2_evol.pdf}
%\caption{}
\end{subfigure}
\begin{subfigure}[tbhp]{0.6\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{AD-1D-StatComparison_batchfiles_200_test_WD_error_M_1_evol.pdf}
%\caption{}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[tbhp]{0.6\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{AD-1D-StatComparison_batchfiles_200_test_WD_error_M_2_evol.pdf}
%\caption{}
\end{subfigure}
\caption{
Starting from $20$ different initial conditions, we propagate the dynamics of the Advection-Diffusion in the one dimensional space ($d_{\bmx}=1$) with LED $400$ different times, changing the seed up to a final time of $T_f=4000$, which is equivalent to $8000$ steps.
For every runs, we calculate the first two moments of the configuration, M1 and M2.
At each time-step, we have $400$ predicted M1 and M2.
We plot the statistical errors (L1-NHD and Wasserstein distance), between the predicted distributions of M1/M2 and the groundtruth, as function of time.
The mean over all initial conditions is reported.
}
\label{fig:app:AD-1D:statistical_analysis_1}
\end{figure*}

In~\Cref{fig:app:AD-1D:statistical_analysis_2}, we plot how the errors vary with respect to the ratio between the time spent in the macro dynamics (LED latent state) and the micro dynamics $\rho=T_m/T_{\mu}$.
The mode where LED is propagating solely on its latent space is denoted as Latent-LED.
The Latent propagation exhibits the highest errors in all metrics.
However, the propagation on the latent state is two orders of magnitude faster compared to the micro dynamics.
This speed-up is reduced as we spent more time on the micro state, exchanging between latent propagation and micro solver dynamics (decreasing $\rho$), gaining a reduction on the errors in all metrics.
\begin{figure*}[tbhp]
\centering
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth,left]{AD-1D-StatComparison_batchfiles_200_test_L1_hist_error_M_1_mean.pdf}
%\caption{}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{AD-1D-StatComparison_batchfiles_200_test_L1_hist_error_M_2_mean.pdf}
%\caption{}
\end{subfigure}
\hfill
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth,left]{AD-1D-StatComparison_batchfiles_200_test_Speedup.pdf}
%\caption{}
\end{subfigure}
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{AD-1D-StatComparison_batchfiles_200_test_WD_error_M_1_mean.pdf}
%\caption{}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{AD-1D-StatComparison_batchfiles_200_test_WD_error_M_2_mean.pdf}
%\caption{}
\end{subfigure}
\hfill
\begin{subfigure}[tbhp]{0.3\textwidth}
\centering
\includegraphics[width=1.0\textwidth,left]{AD-1D-StatComparison_batchfiles_200_test_Speedup_LOG.pdf}
%\caption{}
\end{subfigure}
\caption{
Starting from $20$ different initial conditions, we propagate the dynamics of the Advection-Diffusion in the one dimensional space ($d_{\bmx}=1$) with LED $400$ different times, changing the seed up to a final time of $T_f=4000$, which is equivalent to $8000$ steps.
For every run, we calculate the first two moments of the configuration, M1 and M2.
At each time-step, we have $400$ predicted M1 and M2.
The bars show the mean (over time and initial conditions) statistical errors (L1-NHD and Wasserstein distance), between the predicted distributions of M1/M2 and the groundtruth.
The self-similar error is plotted for reference~\cite{cao2006accuracy} as errors below this level are statistically insignificant.
We observe due to the iterative prediction on the latent space, Latent-LED exhibits the highest errors in all metrics.
However the Latent-LED is more than two orders of magnitude faster compared to the micro solver.
By spending a reference time $T_{\mu}$ on the fine scale dynamics (particles), we achieve a significant error reduction in all metrics, albeit at the cost of reduced speed-up.
On the other hand, as the multiscale ratio $\rho$ is increased, spending more time in the latent propagation, the errors gradually increase.
}
\label{fig:app:AD-1D:statistical_analysis_2}
\end{figure*}

\fi


\clearpage
\newpage

\subsubsection{Hyper-parameter Tuning}
\label{app:sec:ad1d:hyperparams}
We tuned the hyper-parameters of LED based on a grid search, considering the values of hyper-parameters given in~\Cref{app:tab:hypauto_ad1d} for the Autoencoder, and~\Cref{app:tab:hyprnn_ad1d} for the RNN.
\begin{table}[tbhp]
\caption{Autoencoder hyper-parameters for Advection-Diffusion in 1-D ($d_{\bmx}=1$)}
\label{app:tab:hypauto_ad1d}
\centering
\begin{tabular}{ |c|c|c| } 
\hline
\text{Hyper-parameter} & 
\text{Values} \\  \hline \hline
Number of AE layers & $\{5\}$ \\
Size of AE layers & $\{100 \}$ \\
Activation of AE layers & $\operatorname{tanh}(\cdot)$ \\
Latent dimension & $\{1,2,3,4,5,6,7,8,9,10,12,16,18,22,24,28,32,64 \}$ \\
Residual connections & True \\
Variational & True/False \\
Permutation Invariant Layer $d_p$& $\{ 200, 1001\}$ \\
Number of MD kernels $K$& $\{ 4\}$ \\
Hidden units of MD decoder & $\{ 50\}$ \\
Input/Output data scaling & Min-Max in $[0,1]$ \\
Noise level in the data & $\{0, 1,  10 \}$ $(\permil)$ \\
Weight decay rate & $\{0.0, 0.0001 \}$ \\
Batch size& $32$ \\
Initial learning rate & $0.001$ \\
\hline
\end{tabular}
\end{table}
\begin{table}[tbhp]
\caption{LED-RNN hyper-parameters for Advection-Diffusion in 1-D ($d_{\bmx}=1$)}
\label{app:tab:hyprnn_ad1d}
\centering
\begin{tabular}{ |c|c|c| } 
\hline
\text{Hyper-parameter} & 
\text{Values} \\  \hline \hline
Number of AE layers & $\{5\}$ \\
Size of AE layers & $\{100 \}$ \\
Activation of AE layers & $\operatorname{tanh}(\cdot)$ \\
Latent dimension & $\{1, 2\}$ \\
Residual connections & True \\
Variational & True/False \\
Permutation Invariant Layer $d_p$& $\{ 200\}$ \\
Number of MD kernels $K$& $\{ 4\}$ \\
Hidden units of MD decoder & $\{ 50\}$ \\
Input/Output data scaling & Min-Max in $[0,1]$ \\
Noise level in the data & $\{0\}$ \\
Weight decay rate & $\{0.0001 \}$ \\
Batch size& $32$ \\
Initial learning rate & $0.001$ \\
BBTT Sequence length & $\{100 \}$ \\
Hidden state propagation length & $500$ \\
RNN cell type & $\{ \operatorname{lstm}, \operatorname{gru} \}$ \\
Number of RNN layers & $\{1\}$ \\
Size of RNN layers & $\{100\}$ \\
Activation of RNN Cell & $\operatorname{tanh}(\cdot)$ \\
\hline
\end{tabular}
\end{table}


==> section-conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     CONCLUSION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
\label{sec:app:discussion}

We have presented a novel data-driven framework for learning the effective dynamics (LED) and performing multiscale modeling on both stochastic and deterministic dynamical systems, extending the equation-free formalism with state of the art deep learning methods.
LED is utilizing deep autoencoders to compress the high-dimensional state to a few effective degrees of freedom in a latent space representation.
An RNN is utilized to forecast the dynamics on this latent representation.
In stochastic systems, a Mixture Density decoder is probabilistically mapping the reduced order latent space in the high-dimensional state space.

In systems where evolving the high-dimensional state dynamics based on first principles (solvers, equations, etc.) is computationally expensive, or time consuming, LED can accelerate the simulation by propagating on the latent space and then upscaling to high-dimensional system state with the decoder, when necessary.
We demonstrate that LED can be up to three orders of magnitude faster than micro scale solvers, extending the simulation times that are possible with the solvers based on first principles.
Moreover, LED can be operated in a multiscale fashion, switching between propagation of the latent dynamics, and evolution of the micro dynamics, achieving lower error at the cost of reduced speed-up.
In this way, a trade-off between accuracy and speed-up may be achieved. 
The efficiency of the proposed approach is evaluated on a stochastic dynamical system composed of $1000$ particles following the Advection-Diffusion dynamics (AD), the FitzHugh-Nagumo (FHN), the chaotic Kuramoto-Sivashinsky (KS) equation, the stochastic dynamics of a molecule of alanine dipeptide in water, and the von K\'arm\'an vortex street in a flow behind a cylinder at $Re=100$ and $Re=1000$.

LED efficiently uncovers the effective dynamics in the AD equation, capturing the distribution of the positions of the particles with low error, while being two orders of magnitude faster than the micro scale solver.
By utilizing the proposed multiscale forecasting scheme, the statistical error is decreased as more time is spent evolving the particle dynamics, and the less time spent on the latent space of LED, albeit at the cost of lower computational savings.

The efficiency of LED is evaluated in forecasting the evolution of the densities of the activator and the inhibitor in the FHN equation, and compared it with equation-free variants based on uncovering a PDE model on the coarse level.
LED variants exhibit one order of magnitude lower MNAD error on both predicted densities, while being two orders of magnitude faster compared to the Lattice Boltzmann method considered as the micro scale solver.
The multiscale approach is evaluated on the FHN, demonstrating that the error can be further reduced by utilizing the solver for some portion of the forecasting time, at the cost of reduced speed-up, achieving a compromise between the desired accuracy and execution time.

In the chaotic KS equation at spatial extend $L=22$, LED efficiently uncovers an $d_z=8$ dimensional reduced order manifold in the dynamics.
Even though LED is propagating the dynamics on this reduced order space, it is able to reproduce the statistics of the high-dimensional space at the output of the decoder accurately and reproduce the long-term behavior (climate) of the KS equation for a large forecasting horizon, while being two orders of magnitude faster.

LED can efficiently capture the long-term statistics in complex molecular dynamics, while regions in the latent space are mapped to meta stable states, as demonstrated in the alanine dipeptide example.
In our recent work~\cite{vlachas2021accelerated}, we demonstrate that LED also captures the time-scales between the meta stable states and samples realistic protein configurations while being three orders of magnitude faster than the MD solver.

Last but not least, LED can map the Navier-Stokes dynamics of the von K\'arm\'an vortex street in a flow behind a cylinder at $Re=100$ and $Re=1000$, solved with a Finite Element Method, in a low dimensional non-liner latent embedding, allowing for accurate long-term forecasts.
LED is four to five times faster than the FEM solver, and can reproduce global quantities like the drag coefficient.

Future research efforts focus on the scalability of the approach to more high-dimensional problems.
Further study is required in the analysis of the latent space that the LED autoencoders are learning.
In this work, there is no guarantee that the components of the latent space are independent.
Future work can be targeted at unraveling a statistically independent latent space.
The latent space can be used to efficiently classify various regions of the state space of each system and assist in understanding the different regions and their properties.

In summary, LED identifies and propagates the effective dynamics of dynamical systems with multiple spatiotemporal scales providing significant computational savings.
LED provides a systematic way of trading between speed-up and accuracy for a multiscale system by switching between propagation of the latent dynamics, and evolution of the original equations, iteratively correcting the statistical error at the cost of reduced speed-up.
The present methodology can be deployed both in problems described by first principles as well as for problems where only data are available for either the macro or microscale descriptions of the system.
Finally, by providing a bridge between data driven and first principles models LEDs open new horizons for the effective simulations of complex multiscale systems. 



